On $b$-Matching and Fully-Dynamic Maximum $k$-Edge Coloring

Given a graph $G$ that is modified by a sequence of edge insertions and deletions, we study the Maximum $k$-Edge Coloring problem Having access to $k$ colors, how can we color as many edges of $G$ as possible such that no two adjacent edges share the same color? While this problem is different from simply maintaining a $b$-matching with $b=k$, the two problems are closely related: a maximum $k$-matching always contains a $\frac{k+1}k$-approximate maximum $k$-edge coloring. However, maximum $b$-matching can be solved efficiently in the static setting, whereas the Maximum $k$-Edge Coloring problem is NP-hard and even APX-hard for $k \ge 2$. We present new results on both problems: For $b$-matching, we show a new integrality gap result and for the case where $b$ is a constant, we adapt Wajc's matching sparsification scheme~[STOC20]. Using these as basis, we give three new algorithms for the dynamic Maximum $k$-Edge Coloring problem: Our MatchO algorithm builds on the dynamic $(2+\epsilon)$-approximation algorithm of Bhattacharya, Gupta, and Mohan~[ESA17] for $b$-matching and achieves a $(2+\epsilon)\frac{k+1} k$-approximation in $O(poly(\log n, \epsilon^{-1}))$ update time against an oblivious adversary. Our MatchA algorithm builds on the dynamic $8$-approximation algorithm by Bhattacharya, Henzinger, and Italiano~[SODA15] for fractional $b$-matching and achieves a $(8+\epsilon)\frac{3k+3}{3k-1}$-approximation in $O(poly(\log n, \epsilon^{-1}))$ update time against an adaptive adversary. Moreover, our reductions use the dynamic $b$-matching algorithm as a black box, so any future improvement in the approximation ratio for dynamic $b$-matching will automatically translate into a better approximation ratio for our algorithms. Finally, we present a greedy algorithm that runs in $O(\Delta+k)$ update time, while guaranteeing a $2.16$~approximation factor.

==> 3-static.tex <==
\section{Static Algorithms}\label{sect:static}

In this section, we describe static algorithms for $k$-edge coloring. We give two algorithms: a greedy algorithm, which yields a  $3$-approximation and runs in $O(km)$ time, and an algorithm based on $b$-matchings, that runs in $O(\sqrt{kn} m) $ time and yields a $\frac {k+1} k$-approximation.

\subsection{The Greedy Algorithm}
The Greedy Algorithm works as follows: Let $F$ be the set of edges that could be colored, and first set $F=E$. In each iteration, pick an arbitrary edge from $F$, and try to find a color that is free at both its endnodes. If such a color exists, color the edge with that color. Then remove that edge from $F$. The algorithm terminates when $F=\varnothing$.

\begin{theorem}
The Greedy Algorithm runs in $O(km)$ time and is a 3-approximation of Maximum Edge Coloring.
\end{theorem}

It is easy to see that the running time of the Greedy Algorithm is indeed $O(km)$: there are $m$ edges to check, and at each node one can maintain an array of the state of each color at that node (free or not). Then at each iteration, one needs to spend $O(k)$ time to find a free color at both endnodes of the edge, and eventually update the arrays.

It remains to see that this strategy indeed gives a $3$-approximation. It is easy to see that this coloring is maximal, in the following sense:

\begin{definition}
Let $G=(V,E)$ be a graph, $k\in \N_+$, and $f:E\mapsto [k]\union \{\bot\}$ a proper partial coloring of the edges of $E$. 
We say that $f$ is maximal if for every uncolored edge $e$, there is no color that is free at both its endpoints.
\end{definition}

The $3$-approximation guarantee is then a direct implication of the following lemma:

\begin{lemma}
    Let $G=(V,E)$ be a graph, $k\in \N_+$, and $f:E\mapsto [k]\union \{\bot\}$ a proper partial coloring of the edges of $E$. If $f$ is maximal, then $f$ is a 3-approximation of Maximum Edge Coloring.
\end{lemma}



\begin{proof}
Let $H^*$ be the edges of $G$ colored by $f^*$, and $H$ the edges of $G$ colored by $f$. Assign each $e \in H^* \setminus H$ to its adjacent edge $e' \in H$ such that $f^*(e)=f(e')$. Such an edge exists by maximality of $f$. Each edge in $H$ gets assigned at most $2$ edges from $H^*\setminus H$, one at each of its endnodes (and no more, otherwise $f^*$ wouldn't be a proper coloring. This shows that $\card{H^* \setminus H} \le 2 \card H$ and thus $\card {H^*} \le 3\card H$. 
\end{proof}


\subsection{The $k$-Matching Based Algorithm}
The $k$-matching based algorithm works as follows: first, compute a maximum $k$-matching. This $k$-matching has maximum degree $k$, so we can then find a total coloring of that $k$-matching using $k+1$ colors, and finally discard all edges of the color least used.
To the best of our knowledge, this approach was first described by Feige, Ofek, and Wieder~\cite{originalpaper}.
\kh{Feige et al. describe the very same algorithm, just a bit more general for multigraphs. I don't think we need the proof below.}
We use Gabow's $b$-matching algorithm~\cite{gabowbmatch} for solving $k$-matching, and Sinnamon's Algorithm~\cite{DBLP:journals/corr/abs-1907-03201} for coloring the edges.

\begin{theorem}\label{thm:kmatchcoloring}
    The $k$-matching based algorithm runs in $O(\sqrt{kn}m)$ time and is a $\frac {k+1} k$-approximation algorithm of Maximum Edge Coloring.
\end{theorem}

\begin{proof}
This algorithm runs in $O(\sqrt{kn}m)$ time, as Gabow's $b$-matching algorithm takes $O(\sqrt{kn}m)$, and Sinnamon's Algorithm takes $O(m\sqrt{n})$ time. The approximation ratio is guaranteed by the $k$-matching Coloring Theorem, stated and proven below.
\end{proof}

\begin{theorem}[$k$-Matching Coloring]\label{thm:matchingcoloring}
    Let $G$ be a graph and $H$ a subgraph, such that $H$ is an $\alpha$-approximation of  the maximum cardinality `$k$-matching in $G$, for some $\alpha \ge 1$. Let $f$ be a total coloring of $H$ using $k+1$ colors. Then discarding the least used color from $f$ yields an $\alpha \frac {k+1} k$-approximation of the maximum cardinality $k$-edge coloring on $G$.
\end{theorem}

\begin{proof}
    The approximation ratio was first noted by
Feige, Ofek, and Wieder~\cite{originalpaper}.
Indeed, let $f^*$ be the optimal $k$-edge coloring. We know that $f^{*-1}([k])$ is a $k$-matching, and thus cannot be larger than the optimal $k$-matching. Let $f$ be the coloring output by the algorithm. It colors at least $\frac k {k+1}$ edges of $H$, which is larger than $\frac 1 \alpha$ the size of an optimal $k$-matching, and thus $\card{f^{*-1}([k])} \le \frac \alpha {k+1} k \card{f^{-1}([k])}$.
\end{proof}

